On entropy stable temporal fluxes

Entropy-stable (ES) schemes have gained considerable attention over the last decade, especially in the context of turbulent flow simulations using high-order methods. While promising because of their nonlinear stability properties, ES schemes have to address a number of issues to become practical. One of them is how much entropy should be produced by the scheme at a certain level of under-resolution. This problem has been so far studied by considering different ES interfaces fluxes in the spatial discretization only because they can be tuned to generate a certain amount of entropy. In this note, we point out that, in the context of space-time discretizations, the same applies to ES interface fluxes in the temporal direction.

==> Pics/bibtex.tex <==
\bibitem{Lax}
Systems of Conservation Equations with a Convex extension.
\textit{Proceedings of the National Academy of Sciences}, 1971.

@Article{Lax,
  author =	 {K. 0. Friedrichs and P. D. Lax},
  title = {Systems of Conservation Equations with a Convex extension},
  journal =	 {Proceedings of the National Academy of Sciences},
  month =	 may,
  year =	 1971,
}


\bibitem{Lax1}
Hyperbolic Systems of Conservation 
Laws and  the  Mathematical 
Theory of Shock Waves.
\textit{SIAM Regional Conference Lecturers in Applied Mathematics}, 1972.

\bibitem{Kruz}
First-order quasilinear equations in several independent variables.
\textit{Math USSR-Sb}, 1970.

\bibitem{Tadmor0}
Skew-selfadjoint form for systems of conservation laws.
\textit{J. Math. Anal. Appl.}, 1984.

\bibitem{Harten}
On the symmetric form of systems of conservation 
laws with entropy.
\textit{Journal of Comp. Phys.}, 1983.

\bibitem{Tadmor1}
The numerical viscosity of entropy stable schemes for Systems of Conservation Laws
\textit{Mathematics of Computation}, 1987.

\bibitem{LeFloch}
Fully Discrete, Entropy Conservative Schemes of Arbitrary Order
\textit{SIAM J. of Num. Anal.}, 2002.

\bibitem{Tadmor2}
Entropy stability theory
for difference approximations
of nonlinear conservation laws
and related time-dependent problems
\textit{Acta Numerica}, 2003.

\bibitem{Zhong}
Entropy stable approximations of navier-stokes equations with no artificial numerical viscosity, \textit{Journal of Hyperbolic Differential Equations}, 2006.

\bibitem{Barth}
Numerical Methods for Gas Dynamics Systems on Unstructed Meshes, chapter in \textit{An Introduction to Recent Developments in Theory and Numerics for Conservation Laws}, 1998.

\bibitem{Hughes}
A new finite element formulation for computational fluid dynamics: I. Symmetric forms of the compressible Euler and Navier-Stokes equations and the second law of thermodynamics.
\textit{Computer Methods in Applied Mechanics and Engineering}, 1986.

\bibitem{Roe}
Affordable, entropy-consistent, Euler flux functions I. Analytical results. \textit{Journal of Comp. Phys.}.

\bibitem{Chandra}
Kinetic energy preserving and entropy stable finite volume schemes for compressible Euler and Navier-Stokes equations, \textit{arxiv 1209.4994}, 2012.

\bibitem{Roe2}
Approximate Riemann solvers, parameter vectors, and difference schemes,
\textit{Journal of Comp. Phys.}, 1981.

\bibitem{Naterer}
Entropy and the Second Law Fluid Flow and Heat Transfer Simulation, \textit{Journal of thermophysics and heat transfer}, 2003.

\bibitem{Fjordholm}
Arbitrarily High-Order Accurate
Entropy Stable Essentially Nonoscillatory Schemes For Systems of Conservation Laws, \textit{SIAM Journal of Numerical Analysis}, 2012.

\bibitem{Winters}
A Novel Averaging Technique for Discrete Entropy-Stable Dissipation Operators for Ideal MHD, \textit{Journal of Computational Physics},  2017.

\bibitem{Gustafsson}
Time Dependent Problems And Difference Methods, \textit{Pure and Applied Mathematics, Wiley-Interscience Series}, 1995.

\bibitem{Richtmyer}
Difference Methods for Initial-Value Problems, \textit{Interscience Tracts in Pure and Applied Mathematics}, 1967.

\bibitem{Jameson}
Formulation of Kinetic Energy Preserving Conservative Schemes for Gas Dynamics and Direct Numerical Simulation of One-Dimensional Viscous Compressible Flow in a Shock Tube Using Entropy and Kinetic Energy Preserving Schemes, \textit{Journal of Scientific Computing}, 2008.
